Retrieve-Cluster-Summarize: An Alternative to End-to-End Training for Query-specific Article Generation

Query-specific article generation is the task of, given a search query, generate a single article that gives an overview of the topic. We envision such articles as an alternative to presenting a ranking of search results. While generative Large Language Models (LLMs) like chatGPT also address this task, they are known to hallucinate new information, their models are secret, hard to analyze and control. Some generative LLMs provide supporting references, yet these are often unrelated to the generated content. As an alternative, we propose to study article generation systems that integrate document retrieval, query-specific clustering, and summarization. By design, such models can provide actual citations as provenance for their generated text. In particular, we contribute an evaluation framework that allows to separately trains and evaluate each of these three components before combining them into one system. We experimentally demonstrate that a system comprised of the best-performing individual components also obtains the best F-1 overall system quality.

==> introduction-old.tex <==

\vspace{-2em}


\section{Introduction- Old}

%%% Pitch: summarization needs to study effects of upstream systems
Most research on multi-document summarization is performed on benchmarks with a given set of relevant documents to be summarized to resemble a held-out gold summary. The assumption is that such a set of relevant documents can be produced with any retrieval system. However, relevance, cohesiveness, and coverage of search results will affect the quality of the resulting summary. In this paper we depart from this idealized evaluation setting and study complete article generation systems that comprise retrieval, clustering, and summarization components.

%%% Task: article generation (and why helpful)
\textbf{Query-driven Article Generation Task:} We study a task where in response to a broad search query, the system will generate a relevant article (i.e., a long-form summary). The ideal article would cover various relevant subtopics of the information need in a coherent manner as depicted in Figure \ref{fig:example}. Such an article could serve as a means to access information that is complementary to traditional search result rankings. Our system allows users to read a single non-redundant article that fully encompasses the topic of interest---instead of reading multiple documents. This is a benefit for users who seek a general understanding of the topic, require assistance with query reformulation and click decisions, or who are using spoken interfaces.
%% --   

%We identify a use-case of multi-document summarization in which a user's information need is answered by an

%Potential applications of this pipeline include web search, where users generally must select multiple documents from a ranking to read. 

% In order to study the relation between a non-ideal document set and a summarization model, we compare several different methods of retrieving documents for a given query, as well as multiple methods of clustering documents into subtopics prior to summarization. 

\begin{figure}
    \begin{verse}
        
    \textbf{Query: Natural Resources}

Natural resources are classified primarily by their...

Resource extraction is restricted in areas near...

In recent years, resource depletion has become...
    \end{verse}
    \caption{Example article generated in response to a query.}
    \label{fig:example}
\end{figure}

%%% Pitch system that would address task

To generate a relevant article at query-time, we envision a system that retrieves  documents relevant to the query, identifies relevant subtopics via clustering, then uses abstractive multi-document summarization to generate the article. The purpose of the clustering component is to avoid generating incoherent articles that repeatedly switch in-and-out of a subtopic. 

%% retrieve & cluster methods
For 
%document
rankings obtained with different retrieval models, we study the effects of both query-agnostic clustering with Sentence-Bert \cite{reimers2019sentence} as well as query-specific clustering with Q3SM \cite{kashyapi2022query}.

%% summarization system

As a strong summarization system we are experimenting with a pretrained T5 model \cite{raffel2019exploring}, which is applied repeatedly to consolidate subtopic clusters and remove redundancies.

%%% Study 
We study the effect of choices for upstream components retrieval and clustering on the generated article (system evaluation) and compare to evaluation results of each component in isolation. This is made possible by the benchmark creation approach of the TREC Complex Answer Retrieval track \cite{dietz2017trec} that aims to reconstruct human-written Wikipedia pages.\footnote{To avoid confusion we refer to the generated summary as \textsl{article}, but the original Wikipedia entry as \textsl{page}.} Originally the benchmark was created for evaluating a passage retrieval task where queries are derived from Wikipedia section headings, and paragraphs of that section were defined to be relevant. We adapt this approach to use the page title as a query, and define all paragraphs on that page as relevant (we call these \textsl{title-qrels}). A similar idea is used to derive a benchmark for query-specific clustering of paragraphs according to top-level sections of Wikipedia pages \cite{kashyapi2022query}. Likewise we can use the whole content of the Wikipedia page as a gold summary for evaluating how closely the generated article resembles the original human-authored content.

\paragraph{Contributions.}

In this work, we provide:
\begin{itemize}
    \item A joint system for retrieval, clustering, and summarization of query-relevant long-form articles.
    \item An ablation study on the efficacy of different components, which also compares to semi-manual methods.
    \item A study that confirms that component-wise evaluation results agree with the evaluation of the whole system.
\end{itemize}


% \begin{itemize}
%     \item A thorough pipeline with which articles can be written at query-time based around the information need of a user.
%     \item An analysis of said pipeline, with emphasis on finding components that provide high textual similarities to reference articles.
%     \item A discussion of the impact upstream components have on the results of downstream tasks such as multi-document summarization.
% \end{itemize}

\paragraph{Outline.} In Section \ref{sec:related_work} we discuss related work. In Section \ref{sec:approach} we discuss the joint system as well as choices for its retrieval, cluster, and summarization components. In Section \ref{sec:eval} we describe the evaluation of the system and discuss results in Section \ref{sec:results} before concluding the paper.


\progress{End of Page 1}
